Differentially Private Decentralized Learning with Random Walks

The popularity of federated learning comes from the possibility of better scalability and the ability for participants to keep control of their data, improving data security and sovereignty. Unfortunately, sharing model updates also creates a new privacy attack surface. In this work, we characterize the privacy guarantees of decentralized learning with random walk algorithms, where a model is updated by traveling from one node to another along the edges of a communication graph. Using a recent variant of differential privacy tailored to the study of decentralized algorithms, namely Pairwise Network Differential Privacy, we derive closed-form expressions for the privacy loss between each pair of nodes where the impact of the communication topology is captured by graph theoretic quantities. Our results further reveal that random walk algorithms tends to yield better privacy guarantees than gossip algorithms for nodes close from each other. We supplement our theoretical results with empirical evaluation on synthetic and real-world graphs and datasets.

==> avg.tex <==

\section{Random walks for averaging}

We consider the estimation of the mean of all nodes private values. If the values are supposed to be constant with the time, from the local differential point of view, there is no need to add different noises at the different iterations. Doing so would increase the privacy leakage, as the different noise are independent, whereas otherwise the different steps can be seen as post-processing. At the local differential privacy level, \cref{algo:rw_average} is thus optimal: next contribution of a given node can be seen as post-processing of the first contribution. However, if we want to use amplification by iteration coming from the noise of the other nodes, this noise should remain private during all the algorithm, which leads to the need of fresh noise at each contribution. In this case, we need the latter algorithm \cref{algo:allnoisy_average}.

\begin{algorithm}[H]
    \DontPrintSemicolon
    \KwIn{local values $(x_v)_{v\in V}$ to average, gossip matrix $W$ on a graph $G$, in $T$ iterations, noise variance $\sigma^2$, starting node $v$}
    \For{all nodes $v$ in parallel}{
        $x_v \leftarrow x_v + \eta_v$ where $\eta_v \sim \gau{\sigma^2 I}$\;
    }
    \For{$t = 0$ to $T-1$}{
        Draw $u$ in the set of neighbors $N_v$\;
        Send token to $u$\;
        Update token value $S \leftarrow S \frac{t}{t+1} + \frac{x_u}{t+1}$\;
        $v \leftarrow u$\;
    }
    \caption{\textsc{Private random walk averaging}}
    \label{algo:rw_average}
\end{algorithm}

\begin{algorithm}[H]
    \DontPrintSemicolon
    \KwIn{local values $(x_v)_{v\in V}$ to average, gossip matrix $W$ on a graph $G$, in $T$ iterations, noise variance $\sigma^2$, starting node $v$}

    \For{$t = 0$ to $T-1$}{
        Draw $u$ in the set of neighbors $N_v$\;
        Send token to $u$\;
        Update token value $S \leftarrow S \frac{t}{t+1} + \frac{x_u + \eta}{t+1}$ where $\eta \sim \gau{\sigma^2 I}$\;
        $v \leftarrow u$\;
    }
    \caption{\textsc{Private random walk averaging}}
    \label{algo:allnoisy_average}
\end{algorithm}

For analyzing the utility, we need to quantify how fast the average converges to the average of all nodes. In fact, the difference between the time spends in each node since the beginning of a walk and the time predicted by the stationary distribution of the Markov chain is a known quantity of graph theory, the Cesaro Mixing time. We first recap the definition of Mixing time and some property.

\begin{defn}
    The mixing time $\tmix(\eps)$ of a Markov chain is the time needed for the walk to be close to a factor $\eps$ of its assymptotic behavior:

    \begin{equation}
        \tmix(\eps) = \min \left(t: \max_v \norm{P_v^t - \pi}_{TV} \leq \eps\right)
    \end{equation}
\end{defn}

When $\eps$ is not given, it is taken $\eps=1/4$. In fact, having this value is enough, as the following property holds:
\begin{equation}
    \tmix(\eps) \leq \lceil \log_2 \eps^{-1} \rceil t_{mix}
\end{equation}

\begin{defn}
    The Cesaro Mixing time $t_{Ces}$ of a Markov chain is defined as 
    \begin{equation}
        t_{Ces}(\eps) = \min \left(t: \norm{\max_v \frac{1}{t} \sum_{s=1}^t P_v^s -\pi }_{TV} \leq \eps  \right)
    \end{equation}
\end{defn}

It can be proven that the two quantities are related. In particular, we have $t_{Ces} \leq 7 T_{mix}$. More generally, Cesaro mixing time can be bound by any stationary time, in particular hitting times $t_{Ces} \leq 4 t_{hit} +1$: Reciprocally, for 
\begin{equation}
    t_{\text {stop }}=\max _{x \in \mathcal{X}} \inf \left\{\mathbf{E}_x\left(\tau^x\right): \tau^x \text { is a stopping time with } \mathbf{P}_x\left\{X_{\tau^x}=\cdot\right\}=\pi\right\}
\end{equation}
we can lower bound for reversible markov chain $t_{stop}\leq 4 t_{Ces} + 1$.

\edwige{Unsure here what is the best bound to use with close formula to compute the stopping time... Plus, if I understand correctly, for nodes maximizing the hitting time, as the expected commuted time is twice bigger, it mean that we expect two commute for the whole walk to converge}

\subsection{Privacy analysis}

For a walk starting in $v$, the privacy loss towards node $u$ can be computed using the weak convexity of Renyi Divergence:

\begin{lm}[Renyi convexity]
    Let $\mu_{1}, \ldots, \mu_{n}$ and $\nu_{1}, \ldots, \nu_{n}$ be probability
    distributions over some domain $\mathcal{Z}$ such that for all $i \in[n], 
    \mathrm{D}_{\alpha}\left(\mu_{i} \| \nu_{i}\right) \leq c /(\alpha-1)$ for
    some $c \in(0,1]$. Let $\rho$ be a probability distribution over $[n]$ and denote by $\mu_{\rho}\left(\right.$ or $\left.\nu_{\rho}\right)$ the probability distribution over $\mathcal{Z}$ obtained by sampling i from $\rho$ and then outputting a random sample from $\mu_{i}$ (respectively, $\nu_{i}$). Then
    \begin{equation}
    \mathrm{D}_{\alpha}\left(\mu_{\rho} \| \nu_{\rho}\right) \leq(1+c) \cdot \underset{i \sim \rho}{\mathbb{E}}\left[\mathrm{D}_{\alpha}\left(\mu_{i} \| \nu_{i}\right)\right]
    \end{equation}
\end{lm}


Partitioning according to the length of the walk, we can write the privacy guarantee depending on  $T$ the total number of steps and $\beta$ a function bounding the privacy loss occurring for seeing the token $i$ steps after the node contribution:
\begin{equation}
    \eps_{u \rightarrow v} \leq (1+c) \sum_{i=1}^T \Pro(u \rightarrow v \text{ after } k \text{
steps}) \beta(i)
\end{equation}

The goal in then to instantiate the formula with known bound of privacy. It is easy to see that the biggest term is the first one, bounded by $\alpha / 2 \sigma^2$. Hence, we have the constraint $\sigma \geq \sqrt{\alpha(\alpha - 1)/2}$ for all the next results of this document.

Using the gossip matrix to express the probabilities, taking $c=1$ the previous expression can be rewritten as:

\begin{equation}
\eps_{u \rightarrow v} \leq \sum_{i=1}^T W_{uv}^i 2\beta(i)
\end{equation}

Here, as Gaussian noises from the various nodes add up, we can use $\beta(i) = \frac{\alpha}{2\sigma^2 i}$. 
Using simple algebra, we can upper bound the previous expression by a closed form.

\begin{thm}
    Let consider a fixed graph as described in the setting. After $T$ iterations, the privacy loss of a contribution from node $u$ to $v$ is bounded by the following privacy loss:
        \begin{equation}
            \eps_{u \rightarrow v} \leq \frac{\alpha \ln(T)}{\sigma^2 n} - \frac{\alpha}{\sigma^2}\ln(I-W + \frac{1}{n}\one\transp{\one})_{uv}
        \end{equation}
\end{thm}

\begin{proof}
    
\begin{equation}
    \eps_{u \rightarrow v} = \frac{1}{n} \sum_{i=1}^T \frac{\alpha}{\sigma^2 i} + \sum_{i=1}^T \left(\sum_{j=2}^n \lambda_j^i\phi(j)\transp{\phi(j)}\frac{\alpha}{\sigma^2 i}\right)_{uv}
\end{equation}

We can simplify the formula further, noticing that $\sum_{i=1}^\infty {\lambda_j^i}/{i} = - \ln(1-\lambda_j)$ leading to the following result:
\begin{equation}
    \eps_{u \rightarrow v} \leq \frac{\alpha}{\sigma^2} \left(\frac{\ln(T)}{n} - \sum_{j=2}^n \phi(j)_u\transp{\phi(j)_v} \ln(1-\lambda_j) \right)
\end{equation}
\end{proof}


\begin{rmk}
    The previous equation makes appears a weighted sum of the powers of the communication matrix. This combination is already used in other graph application. In particular, changing the coefficient of $i$-th iterate from $\frac{1}{i}$ to $\frac{1}{i!}$ gives the notion of communicability.
\end{rmk}

Thus, for computing the average of private values, we thus have close form both from the privacy and the utility of the random walk.

\edwige{Here I have some issue to compute the privacy utility trade-off.}
The minimization is is $\eps + \sigma \sqrt{4t_{mix}\log(1/\eps)}$ which seems to require constraint on the parameter to have a global minima, which sounds counterintuitive for me. 


